Chandra, HST/STIS, NICER, Swift, and TESS Detail the Flare Evolution of the Repeating Nuclear Transient ASASSN-14ko

ASASSN-14ko is a nuclear transient at the center of the AGN ESO 253-G003 that undergoes periodic flares. Optical flares were first observed in 2014 by the All-Sky Automated Survey for Supernovae (ASAS-SN) and their peak times are well-modeled with a period of $115.2^{+1.3}_{-1.2}$ days and period derivative of $-0.0026 \pm 0.0006$. Here we present ASAS-SN, Chandra, HST/STIS, NICER, Swift, and TESS data for the flares that occurred in December 2020, April 2021, July 2021, and November 2021. The HST/STIS UV spectra evolve from blue shifted broad absorption features to red shifted broad emission features over $\sim$10 days. The Swift UV/optical light curves peaked as predicted by the timing model, but the peak UV luminosities varied between flares and the UV flux in July 2021 was roughly half the brightness of all other peaks. The X-ray luminosities consistently decreased and the spectra became harder during the UV/optical rise but apparently without changes in absorption. Finally, two high-cadence TESS light curves from December 2020 and November 2018 showed that the slopes during the rising and declining phases changed over time, which indicates some stochasticity in the flare's driving mechanism. ASASSN-14ko remains observationally consistent with a repeating partial tidal disruption event, but, these rich multi-wavelength data are in need of a detailed theoretical model.

==> rise_decline_fits.tex <==
\begin{tabular*}{0.93\textwidth}{l l l l l}
\toprule
 & &  \textbf{Power-Law Decline}&  & \\
 %& & \pbox{33mm}{ \textbf{Power-Law Decline November 2018}} &  & \\
\pbox{25mm}{ Fit Start Time\\from Peak (Days)} & \pbox{30mm}{$t_0$ (JD-2458435.26)} & \pbox{40mm}{$h$ (ergs s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)} & $\alpha$ & \pbox{25mm}{$\chi^2$ per dof} \\ 
\hline
  & &  \textbf{November 2018}&  & \\

\hline

3 & $-5.57\pm0.80$  & $-3.74\pm0.80$ & $-1.02\pm0.06$ & 0.98 \\ 
%6 & $-5.57\pm1.70$  & $-7.18\pm3.73$ & $-1.25\pm0.06$ & 0.91 \\
%15 & $29.70\pm3.03$  & $-10.00\pm5.76$ & $-1.38\pm0.13$ & 0.72 \\ 
%20 & $29.70\pm6.23$  & $-10.00\pm10.90$ & $-1.40\pm0.24$ & 0.70 \\ 

\hline

&  & \textbf{December 2020} &  & \\
%\pbox{25mm}{ Fit Start Time\\from Peak (Days)} & \pbox{25mm}{$t_0$ (JD-2459205.60)} & \pbox{40mm}{$h$ (ergs s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)} & $\alpha$ & \pbox{25mm}{$\chi^2$ per dof} \\ 

\hline

3 & $-5.72\pm0.91$  & $-1.87\pm0.33$ & $-0.76\pm0.05$ & 0.97 \\ 
%6 & $29.70\pm1.11$  & $-10.00\pm2.51$ & $-1.35\pm0.06$ & 0.91 \\
%15 & $29.70\pm3.03$  & $-10.00\pm5.76$ & $-1.38\pm0.13$ & 0.72 \\ 
%20 & $29.70\pm6.23$  & $-10.00\pm10.90$ & $-1.40\pm0.24$ & 0.70 \\ 

\toprule

 &  & \textbf{Exponential Decline } & & \\
\pbox{25mm}{ Fit Start Time\\from Peak (Days)} &  \pbox{40mm}{$a$ (ergs s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)} & \pbox{25mm}{$\tau$ (days)} & \pbox{25mm}{$c$ (days)} & \pbox{25mm}{$\chi^2$ per dof} \\
\hline
 &  & \textbf{November 2018 } & & \\
\hline

3 & $0.47\pm0.02$ & $22.55\pm1.20$ & $-0.12\pm0.017$ & 0.52 \\
%6 & $0.22\pm0.001$ & $11.06\pm0.14$ & $0.02\pm0.001$ & 0.60 \\
%15 & $0.13\pm0.001$ & $12.11\pm0.33$ & $0.01\pm0.001$ & 0.56 \\
%20 & $0.09\pm0.001$ & $10.83\pm0.44$ & $0.02\pm0.001$ & 0.55 \\ 
\hline 

&  & \textbf{December 2020} & & \\
\hline

3 & $0.47\pm0.03$ & $33.72\pm3.29$ & $-0.14\pm0.03$ & 0.74 \\
%6 & $0.22\pm0.001$ & $11.06\pm0.14$ & $0.02\pm0.001$ & 0.60 \\
%15 & $0.13\pm0.001$ & $12.11\pm0.33$ & $0.01\pm0.001$ & 0.56 \\
%20 & $0.09\pm0.001$ & $10.83\pm0.44$ & $0.02\pm0.001$ & 0.55 \\ 
\hline 


\end{tabular*}
